On mining complex sequential data by means of FCA and pattern structures

Nowadays data sets are available in very complex and heterogeneous ways. Mining of such data collections is essential to support many real-world applications ranging from healthcare to marketing. In this work, we focus on the analysis of "complex" sequential data by means of interesting sequential patterns. We approach the problem using the elegant mathematical framework of Formal Concept Analysis (FCA) and its extension based on "pattern structures". Pattern structures are used for mining complex data (such as sequences or graphs) and are based on a subsumption operation, which in our case is defined with respect to the partial order on sequences. We show how pattern structures along with projections (i.e., a data reduction of sequential structures), are able to enumerate more meaningful patterns and increase the computing efficiency of the approach. Finally, we show the applicability of the presented method for discovering and analyzing interesting patient patterns from a French healthcare data set on cancer. The quantitative and qualitative results (with annotations and analysis from a physician) are reported in this use case which is the main motivation for this work. Keywords: data mining; formal concept analysis; pattern structures; projections; sequences; sequential data.

==> tex/fig-AWD-times.tex <==
\newcommand{\drawAWDTimes}{
\drawScatter{User Count}{Time ($s$)}{
	\addPlot{mark=+}{0}{2}{$l=3$}{web-data/data.3.st}
	\addPlot{mark=x}{0}{2}{$l=4$}{web-data/data.4.st}
	\addPlot{mark=diamond}{0}{2}{$l=5$}{web-data/data.5.st}
}
}

\begin{figure}
	\centering
	\drawAWDTimes
	\vspace{-0.5cm}
	\caption{Execution time w.r.t a number of added users.}
	\label{fig:AWD-times}
\end{figure}

==> tex/fig-PMT-lattice.tex <==
\newcommand{\drawPMTLattice}{
	\drawScatter{Patients Count}{Lattice Size}{
		\addPlot{mark=+}{0}{1}{$l=2$}{pmt/data.2.st}
		\addPlot{mark=x}{0}{1}{$l=3$}{pmt/data.3.st}
		\addPlot{mark=asterisk}{0}{1}{$l=4$}{pmt/data.4.st}
		\addPlot{mark=diamond}{0}{1}{$l=5$}{pmt/data.5.st}
		\addPlot{mark=triangle}{0}{1}{$l=6$}{pmt/data.6.st}
	}
}

\begin{figure}
	\centering
	\drawPMTLattice
	\caption{Dependence of the lattice size on the number of patients for the PMT database.}
	\label{fig:PMT-lattice}
\end{figure}

==> tex/fig-PMT-times.tex <==
\newcommand{\drawPMTTimes}{
\drawScatter{Patients Count}{Time ($s$)}{
	\addPlot{mark=+}{0}{2}{$l=2$}{pmt/data.2.st}
	\addPlot{mark=x}{0}{2}{$l=3$}{pmt/data.3.st}
	\addPlot{mark=asterisk}{0}{2}{$l=4$}{pmt/data.4.st}
	\addPlot{mark=diamond}{0}{2}{$l=5$}{pmt/data.5.st}
	\addPlot{mark=triangle}{0}{2}{$l=6$}{pmt/data.6.st}
}
}

\begin{figure}
	\centering
	\drawPMTTimes
	\vspace{-0.5cm}
	\caption{Execution time w.r.t a number of added patients.}
	\label{fig:PMT-times}
\end{figure}

==> tex/fig-result-stats.tex <==
\begin{figure*}
	\centering
	\begin{subfigure}[t]{0.415\columnwidth}
		\centering
		\includegraphics[width=\columnwidth]{./plots/time.png}
		\caption{Working time}
		\label{fig:time}
	\end{subfigure}
	\begin{subfigure}[t]{0.5\columnwidth}
		\centering
		\includegraphics[width=\columnwidth]{./plots/concept.pdf}
		\caption{Concepts}
		\label{fig:concept}
	\end{subfigure}
	\begin{subfigure}[t]{0.5\columnwidth}
		\centering
		\includegraphics[width=\columnwidth]{./plots/stable.pdf}
		\caption{Stable concepts}
		\label{fig:stable}
	\end{subfigure}
	\caption{
		Parameters of the result for different projections.
	}
	\label{fig:result-stats}
\end{figure*}

==> tex/settings-template.tex <==
\newcommand{\putBibliography}{
	\bibliography{./library}
}


==> tex/tbl-AWD-concepts.tex <==
\begin{table}
	\centering
	\resizebox{0.8\columnwidth}{!}{
	\begin{tabular}{c|c|c@{ }c}
	& Intent & \multicolumn{2}{|c}{Extent} \\
	\hline
	$c_1$
	& $\seq{FP\+News\+FP}$ & 25111 & ($2.5\%$) \\
	$c_2$
	& $\seq{FP\+Business\+FP}$ & 16584 & ($1.6\%$) \\
	$c_3$
	& $\seq{Misc\+OnAir\+Misc\+OnAir\+Misc}$ & 6660 & ($0.6\%$) \\
	\hline	
	\end{tabular}
	}
	\caption{Some interesting concepts for the AWD database}
	\label{tbl:AWD-concepts}
\end{table}

==> tex/tbl-PMT-concepts.tex <==
\begin{table}
	\centering
	\resizebox{\columnwidth}{!}{
	\begin{tabular}{c|c|c@{ }c}
		& Intent & \multicolumn{2}{|c}{Extent} \\
		\hline
		$c_1$
		& $\seq{\set{D_\text{Chemotherapy}}*8}$ & 284 & ($28\%$) \\
		$c_2$
		& $\seq{\set{D_\text{Device Adj.}\+P_\text{Artery Catheter}}\+\set{D_\text{Chemotherapy}}*12}$ & 74 & ($7\%$) \\
		$c_3$
		& $\seq{\set{P_\text{Chest Radiography}}*2}$ & 189 & ($19\%$) \\
		\hline
	\end{tabular}
	}
	\caption{Some interesting concepts of the PMT database}
	\label{tbl:PMT-concepts}
\end{table}

==> tex/tbl-PMT-ex-patients.tex <==
\begin{table}
	\centering
	\resizebox{\columnwidth}{!}{
	\begin{tabular}{l|l}
	Patient & Medical Trajectory \\
	\hline
	
	$p^1$ & $\seq{\set{H_1\+R_1\+P_1\+P_2\+P_3}\+\set{H_2\+R_2}}$\\
	$p^2$ & $\seq{\set{H_3\+R_1\+P_4}\+\set{H_3\+R_3\+P_5}}$\\
	$p^3$ & $\seq{\set{H_4\+R_1\+P_2\+P_6}\+\set{H_5\+R_3\+P_1\+P_4}\+\set{H_5\+R_3}*14}$\\
	$p^4$ &
	$\seq{\set{H_1,R_1,P_2,P_3}\+\set{H_1,R_3}*3\+\set{H_1,R_3,P_4}\+\set{H_1,R_3}*3}$\\
	$p^5$ & 
	$\seq{\set{H_2,R_2,P_1,P_3}\+\set{H_1,R_3,P_4}*4}$ \\
	\hline
	\end{tabular}
	}
	\caption{Examples of sequential data in PMT database.}
	\label{tbl:PMT-ex-patients}
\end{table}

==> tex/tbl-PMT-results.tex <==
\begin{table}
	\centering
	\resizebox{\columnwidth}{!}{
	\begin{tabular}{c|cccccc} 
		Projection 
		& No & $l=2$ & $l=3$ & $l=4$ & $l=5$ & $l=6$ \\
		\hline
		Time($s$)
		& $>1.4*10^5$ & $4510$ & $3878$ & $3722$ & $3435$ & $3120$ \\
		Lattice 
		& $>2.8*10^6$ & $554332$ & $271166$ & $189353$ & $137912$ & $100492$ \\
		\hline
	\end{tabular}
	}
	\caption{The processing time and the lattice size of experiments on the PMT database for different projections}
	\label{tbl:PMT-results}
\end{table}

==> tex/tbl-PMT-stats.tex <==
\begin{table}
\centering
	\begin{tabular}{c|c|c|c|c|c|c}
		\hline
		Patients & Max. Length & Mean Length & $|G|$ & $|T|$ & $|R|$ & $|P|$ \\
		$2618$ & $28$ & $3.65$ & $304$ & $6$ & $1939$ & $723$ \\
		\hline
	\end{tabular}
	\caption{Parameters of the PMT dataset}
	\label{tbl:PMT-stats}
\end{table}

==> tex/tbl-ips-example.tex <==
\begin{table}
\centering
\begin{minipage}{0.33\columnwidth}
	\centering
	\resizebox{\columnwidth}{!}{
	\begin{tabular}{l|ccc}
		Obj\textbackslash Attrs & $m_1$ & $m_2$ & $m_3$ \\
		\hline
		$g_1$ & $[1,3]$ & $[3,5]$ & $[2,4]$\\
		$g_2$ & $[5,7]$ & $[4,6]$ & $[2,5]$\\
		$g_3$ & $[1,9]$ & $[2,7]$ & $[6,6]$\\
		\hline
	\end{tabular}
	}
	\captionof{table}{Example of an Interval Pattern Structure.}
	\label{tbl:ips-example}
\end{minipage}
\begin{minipage}{0.65\columnwidth}
	\centering
	\resizebox{\columnwidth}{!}{\putIPSLattice}
	\captionof{figure}{The concept lattice for the context in Table~\ref{tbl:ips-example}.}
	\label{fig:ips-example}
\end{minipage}
\end{table}


==> tex/tbl-result-concepts.tex <==
\begin{table*}[t]
	\centering
	\caption{Interesting concepts, for different projections. \texttt{Chemo} is chemotherapy, \texttt{Ch.Prep} is preparation for chemotherapy, \texttt{App.} is an operation for appendicitis.}
%	\resizebox{\columnwidth}{!}{
	\begin{tabular}{r||c|c|c|c}
		\hline
		\# & Projection & Intent & Stab. Rank & Support \\
		\hline
		$1$ & \pRiPsII & $\seq{\el{Cancer}{}\+\el{Chemo}{}}$ & $1$ & $452$ \\
		$2$ & \pRiPsII & $\seq{\el{Cancer}{App.}\+\el{Ch.Prep}{}\+\el{Chemo}{}}$ & $4$ & $293$ \\
		$3$ & \pRiPsIII & $\seq{\el{Cancer}{App.}\+\el{Ch.Prep}{}\+\el{Chemo}{}}$ & $2$ & $293$ \\
		$4$ & \pRiPIsIII & $\seq{\el{Cancer}{}*1\+\el{Ch.Prep}{}*1\+\el{Chemo}{}*[8,24]}$ & $4$ & $193$ \\
		$5$ & \pGiRisIII & $\seq{\elnP{Bourgogne,Cancer}\+\elnP{Bourgogne,Ch.Prep}\+\elnP{A~clinic~in~Dijon,Chemo}} $ & $5$ & $29$ \\
		\hline
	\end{tabular}
%	}
	\label{tbl:result-concepts}
\end{table*}

==> tex/tbl-result-stats.tex <==
\begin{table}
	\centering
	\begin{tabular}{l|cc|cc|cc}
		\hline
		Projection & \pRiPsII & \pRiPsIII & \pRiPIsII & \pRiPIsIII & \pGiRisII & \pGiRisIII \\
		\hline
		Time ($s$)          & $18$    & $8$    & $417$     & $15$ & $10$ & $6$ \\
		\#Concepts (1000)             & $34.7$ & $8.67$ & $1856$ & $93.2$ & $4.2$ & $2.2$ \\
		\#($Stab \geq 0.97$) & $615$  & $192$  & $1117$    & $311$ & $131$ & $45$ \\
		\hline
	\end{tabular}
	\caption{Parameters of the result for different projections.}
	\label{tbl:result-stats}
\end{table}
